Predicting Crop Yield With Machine Learning: An Extensive Analysis Of Input Modalities And Models On a Field and sub-field Level

We introduce a simple yet effective early fusion method for crop yield prediction that handles multiple input modalities with different temporal and spatial resolutions. We use high-resolution crop yield maps as ground truth data to train crop and machine learning model agnostic methods at the sub-field level. We use Sentinel-2 satellite imagery as the primary modality for input data with other complementary modalities, including weather, soil, and DEM data. The proposed method uses input modalities available with global coverage, making the framework globally scalable. We explicitly highlight the importance of input modalities for crop yield prediction and emphasize that the best-performing combination of input modalities depends on region, crop, and chosen model.

==> tables/data_sources.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{cllcccc}
\hline
\multicolumn{1}{l}{\textbf{Data   Source}} &
  \multicolumn{1}{c}{\textbf{Product}} &
  \multicolumn{1}{c}{\textbf{Name}} &
  \textbf{Unit} &
  \textbf{Temporal Resolution} &
  \textbf{Resolution} &
  \textbf{Source} \\ \hline
\multicolumn{1}{l}{Imagery} &
  \multicolumn{1}{c}{Sentinel-2} &
  \multicolumn{1}{c}{S2} &
  \textbf{} &
  yes &
  10m &
  ecmwf \\ \hline
\multirow{}{}{Weather}   & Precipitation                             & Total Precipitation & m          & yes & 10km & ecmwf     \\
                           & Max   Temperature                         & 2m temperature      & K          & yes & 10km & ecmwf     \\
                           & Min   Temperature                         & 2m temperature      & K          & yes & 10km & ecmwf     \\
                           & Average   Temperature                     & 2m temperature      & K          & yes & 10km & ecmwf     \\ \hline
\multirow{}{}{Soil}      & Soil Organic carbon                       & soc                 & dg/kg      & no  & 250m & Soilgrids \\
                           & Nitrogen                                  & nitrogen            & cg/kg      & no  & 250m & Soilgrids \\
                           & Cation   exchange capacity                & cec                 & mmol(c)/kg & no  & 250m & Soilgrids \\
                           & Clay                                      & clay                & g/kg       & no  & 250m & Soilgrids \\
                           & Silt                                      & silt                & g/kg       & no  & 250m & Soilgrids \\
                           & Sand                                      & sand                & g/kg       & no  & 250m & Soilgrids \\
                           & Soil pH                                   & phh20               & pHx10      & no  & 250m & Soilgrids \\
                           & Volumetric   fraction of course fragments & cfvo                & cm3/dm3    & no  & 250m & Soilgrids \\ \hline
\multirow{}{}{Elevation} & DEM                                       & dem                 & m          & no  & 250m & SRTM      \\
                           & Slope                                     & slope radians       & radians    & no  & 250m & SRTM      \\
                           & Curvature                                 & curvature           & 1/100m     & no  & 250m & SRTM      \\
                           & Aspect                                    & aspect              & deg        & no  & 250m & SRTM      \\
                           & Topographic   Wetness Index               & twi                 &            & no  & 250m & SRTM      \\ \hline
\end{tabular}

